Doubly Robust Conformalized Survival Analysis with Right-Censored Data

We present a conformal inference method for constructing lower prediction bounds for survival times from right-censored data, extending recent approaches designed for more restrictive type-I censoring scenarios. The proposed method imputes unobserved censoring times using a machine learning model, and then analyzes the imputed data using a survival model calibrated via weighted conformal inference. This approach is theoretically supported by an asymptotic double robustness property. Empirical studies on simulated and real data demonstrate that our method leads to relatively informative predictive inferences and is especially robust in challenging settings where the survival model may be inaccurate.

==> tables/table_data_cox_alpha_0.1_small.tex <==
\begin{table}[!h]
\centering
\caption{Caption \label{tab:1}}
\centering
\begin{tabular}[t]{ccc}
\toprule
Method & Estimated Coverage & Mean LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.89 (0.89--0.89}) & 320.96\\
\hspace{1em}Naive CQR & 0.90 (0.90--0.91) & 299.68\\
\hspace{1em}KM Decensoring & 0.90 (0.90--0.90) & 308.78\\
\hspace{1em}DR-COSARC & 0.91 (0.90--0.91) & 288.30\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.89 (0.89--0.90}) & 12.36\\
\hspace{1em}Naive CQR & 0.91 (0.90--0.92) & 11.38\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.90 (0.89--0.90}) & 12.23\\
\hspace{1em}DR-COSARC & 0.90 (0.89--0.91) & 11.87\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.74 (0.64--0.84}) & 28.52\\
\hspace{1em}Naive CQR & 0.94 (0.91--0.97) & 6.97\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.84 (0.77--0.91}) & 17.65\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.84 (0.78--0.90}) & 13.19\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.89 (0.87--0.90}) & 42.41\\
\hspace{1em}Naive CQR & 0.91 (0.90--0.92) & 35.02\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.89 (0.88--0.91}) & 40.55\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.90 (0.88--0.91}) & 38.79\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.85 (0.79--0.90}) & 1198.29\\
\hspace{1em}Naive CQR & 0.94 (0.91--0.96) & 768.98\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.87 (0.82--0.91}) & 1110.57\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.88 (0.85--0.92}) & 1020.75\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.87 (0.85--0.88}) & 8.77\\
\hspace{1em}Naive CQR & 0.91 (0.90--0.92) & 6.55\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.88 (0.86--0.90}) & 8.24\\
\hspace{1em}DR-COSARC & 0.89 (0.88--0.91) & 6.57\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.88 (0.87--0.88}) & 24.64\\
\hspace{1em}Naive CQR & 0.94 (0.94--0.94) & 16.36\\
\hspace{1em}KM Decensoring & 0.89 (0.89--0.90) & 21.93\\
\hspace{1em}DR-COSARC & 0.91 (0.90--0.91) & 18.05\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_cox_alpha_0.2_large.tex <==
\begin{table}[!h]
\centering
\caption{Performance on seven publicly available data sets of different methods for constructing survival LPBs. All methods utilize the same survival model (cox) and aim for 80\% coverage. Since the performance is evaluated on a censored test set, the coverage cannot be evaluated exactly. Instead, we report empirical lower and upper bounds for the true coverage. Values in parentheses represent twice the standard error. Coverage point estimates that are more than two standard errors below the nominal level are highlighted in red. \label{tab:data-cox-large-alpha0.2}}
\centering
\begin{tabular}[t]{ccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Estimated Coverage} & \multicolumn{1}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4}
Method & Point & Lower bound & Upper bound & LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.79 (0.01)} & 0.78 (0.01) & 0.80 (0.01) & 633.67 (10.16)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.82 (0.01)} & 0.81 (0.01) & 0.83 (0.01) & 571.06 (11.80)\\
\hspace{1em}KM Decensoring & \textcolor{black}{0.80 (0.01)} & 0.79 (0.01) & 0.81 (0.01) & 612.62 (11.30)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.80 (0.01)} & 0.80 (0.01) & 0.81 (0.01) & 582.24 (14.35)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.79 (0.01)} & 0.78 (0.01) & 0.80 (0.01) & 19.87 (0.17)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.82 (0.01)} & 0.81 (0.01) & 0.83 (0.01) & 18.30 (0.28)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.79 (0.01)} & 0.78 (0.01) & 0.80 (0.01) & 19.68 (0.29)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.80 (0.01)} & 0.79 (0.01) & 0.81 (0.01) & 19.18 (0.28)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.64 (0.02)} & 0.49 (0.03) & 0.79 (0.02) & 66.18 (9.16)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.86 (0.02)} & 0.80 (0.03) & 0.92 (0.01) & 32.27 (7.94)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.72 (0.03)} & 0.61 (0.05) & 0.83 (0.02) & 51.90 (8.39)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.72 (0.02)} & 0.60 (0.04) & 0.83 (0.02) & 41.67 (6.78)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.76 (0.01)} & 0.73 (0.01) & 0.80 (0.01) & 73.48 (0.88)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.83 (0.00)} & 0.81 (0.01) & 0.86 (0.01) & 59.67 (1.19)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.78 (0.01)} & 0.74 (0.01) & 0.81 (0.01) & 70.45 (1.36)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.78 (0.01)} & 0.75 (0.01) & 0.81 (0.01) & 68.37 (1.41)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.68 (0.01)} & 0.54 (0.02) & 0.81 (0.02) & 1808.76 (46.91)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.87 (0.01)} & 0.80 (0.02) & 0.94 (0.01) & 1117.50 (62.77)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.73 (0.01)} & 0.61 (0.02) & 0.85 (0.02) & 1652.82 (54.37)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.72 (0.02)} & 0.61 (0.03) & 0.83 (0.02) & 1609.90 (52.63)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.73 (0.01)} & 0.68 (0.02) & 0.79 (0.02) & 21.69 (1.13)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.85 (0.01)} & 0.81 (0.02) & 0.88 (0.02) & 13.49 (1.14)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.77 (0.02)} & 0.72 (0.03) & 0.81 (0.02) & 19.37 (1.32)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.78 (0.01)} & 0.75 (0.02) & 0.82 (0.01) & 16.72 (1.22)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & \textcolor{black}{0.79 (0.02)} & 0.78 (0.02) & 0.80 (0.02) & 33.74 (1.35)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.83 (0.02)} & 0.83 (0.03) & 0.84 (0.03) & 29.41 (2.47)\\
\hspace{1em}KM Decensoring & \textcolor{black}{0.80 (0.02)} & 0.79 (0.03) & 0.81 (0.03) & 32.59 (2.49)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.82 (0.02)} & 0.82 (0.02) & 0.83 (0.02) & 29.31 (2.26)\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_cox_alpha_0.2_small.tex <==
\begin{table}[!h]
\centering
\caption{Caption \label{tab:1}}
\centering
\begin{tabular}[t]{ccc}
\toprule
Method & Estimated Coverage & Mean LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.79 (0.78--0.80}) & 633.67\\
\hspace{1em}Naive CQR & 0.82 (0.81--0.83) & 571.06\\
\hspace{1em}KM Decensoring & 0.80 (0.79--0.81) & 612.62\\
\hspace{1em}DR-COSARC & 0.80 (0.80--0.81) & 582.24\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.79 (0.78--0.80}) & 19.87\\
\hspace{1em}Naive CQR & 0.82 (0.81--0.83) & 18.30\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.79 (0.78--0.80}) & 19.68\\
\hspace{1em}DR-COSARC & 0.80 (0.79--0.81) & 19.18\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.64 (0.49--0.79}) & 66.18\\
\hspace{1em}Naive CQR & 0.86 (0.80--0.92) & 32.27\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.72 (0.61--0.83}) & 51.90\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.72 (0.60--0.83}) & 41.67\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.76 (0.73--0.80}) & 73.48\\
\hspace{1em}Naive CQR & 0.83 (0.81--0.86) & 59.67\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.78 (0.74--0.81}) & 70.45\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.78 (0.75--0.81}) & 68.37\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.68 (0.54--0.81}) & 1808.76\\
\hspace{1em}Naive CQR & 0.87 (0.80--0.94) & 1117.50\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.73 (0.61--0.85}) & 1652.82\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.72 (0.61--0.83}) & 1609.90\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.73 (0.68--0.79}) & 21.69\\
\hspace{1em}Naive CQR & 0.85 (0.81--0.88) & 13.49\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.77 (0.72--0.81}) & 19.37\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.78 (0.75--0.82}) & 16.72\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & 0.79 (0.78--0.80) & 33.74\\
\hspace{1em}Naive CQR & 0.83 (0.83--0.84) & 29.41\\
\hspace{1em}KM Decensoring & 0.80 (0.79--0.81) & 32.59\\
\hspace{1em}DR-COSARC & 0.82 (0.82--0.83) & 29.31\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_grf_alpha_0.1_small.tex <==
\begin{table}[!h]
\centering
\caption{Caption \label{tab:1}}
\centering
\begin{tabular}[t]{ccc}
\toprule
Method & Estimated Coverage & Mean LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & 0.91 (0.90--0.91) & 299.15\\
\hspace{1em}Naive CQR & 0.90 (0.90--0.91) & 296.97\\
\hspace{1em}KM Decensoring & 0.90 (0.90--0.90) & 306.27\\
\hspace{1em}DR-COSARC & 0.91 (0.91--0.91) & 286.03\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & 0.90 (0.90--0.91) & 13.10\\
\hspace{1em}Naive CQR & 0.91 (0.90--0.92) & 12.80\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.89 (0.89--0.90}) & 13.70\\
\hspace{1em}DR-COSARC & 0.91 (0.90--0.91) & 12.98\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.84 (0.78--0.90}) & 14.27\\
\hspace{1em}Naive CQR & 0.94 (0.92--0.97) & 3.58\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.84 (0.77--0.91}) & 15.06\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.88 (0.83--0.92}) & 9.74\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & 0.90 (0.89--0.91) & 40.86\\
\hspace{1em}Naive CQR & 0.92 (0.91--0.93) & 37.84\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.89 (0.88--0.90}) & 42.55\\
\hspace{1em}DR-COSARC & 0.90 (0.89--0.91) & 40.10\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & 0.92 (0.89--0.95) & 853.89\\
\hspace{1em}Naive CQR & 0.93 (0.91--0.95) & 784.62\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.85 (0.81--0.90}) & 1035.49\\
\hspace{1em}DR-COSARC & 0.92 (0.89--0.95) & 852.27\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.88 (0.87--0.89}) & 7.58\\
\hspace{1em}Naive CQR & 0.90 (0.89--0.91) & 6.66\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.88 (0.86--0.89}) & 8.03\\
\hspace{1em}DR-COSARC & 0.90 (0.89--0.91) & 6.19\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & 0.93 (0.93--0.93) & 12.35\\
\hspace{1em}Naive CQR & 0.94 (0.94--0.94) & 10.66\\
\hspace{1em}KM Decensoring & 0.90 (0.90--0.90) & 14.47\\
\hspace{1em}DR-COSARC & 0.94 (0.94--0.94) & 10.17\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_grf_alpha_0.2_large.tex <==
\begin{table}[!h]
\centering
\caption{Performance on seven publicly available data sets of different methods for constructing survival LPBs. All methods utilize the same survival model (grf) and aim for 80\% coverage. Since the performance is evaluated on a censored test set, the coverage cannot be evaluated exactly. Instead, we report empirical lower and upper bounds for the true coverage. Values in parentheses represent twice the standard error. Coverage point estimates that are more than two standard errors below the nominal level are highlighted in red. \label{tab:data-grf-large-alpha0.2}}
\centering
\begin{tabular}[t]{ccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Estimated Coverage} & \multicolumn{1}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4}
Method & Point & Lower bound & Upper bound & LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & \textcolor{black}{0.80 (0.01)} & 0.80 (0.01) & 0.81 (0.01) & 567.35 (8.92)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.81 (0.01)} & 0.81 (0.01) & 0.81 (0.01) & 563.05 (12.50)\\
\hspace{1em}KM Decensoring & \textcolor{black}{0.80 (0.01)} & 0.80 (0.01) & 0.80 (0.01) & 576.70 (12.49)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.81 (0.01)} & 0.81 (0.01) & 0.82 (0.01) & 543.45 (9.90)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{black}{0.80 (0.00)} & 0.79 (0.01) & 0.81 (0.01) & 20.59 (0.17)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.82 (0.00)} & 0.81 (0.01) & 0.83 (0.01) & 19.56 (0.30)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.79 (0.01)} & 0.78 (0.01) & 0.81 (0.01) & 20.96 (0.33)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.81 (0.00)} & 0.79 (0.01) & 0.82 (0.01) & 20.12 (0.22)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.69 (0.02)} & 0.56 (0.04) & 0.83 (0.02) & 36.38 (1.45)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.87 (0.02)} & 0.81 (0.03) & 0.93 (0.01) & 12.92 (1.82)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.70 (0.03)} & 0.57 (0.05) & 0.83 (0.02) & 35.96 (2.93)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.74 (0.02)} & 0.63 (0.04) & 0.85 (0.02) & 28.18 (2.77)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.78 (0.00)} & 0.75 (0.01) & 0.81 (0.01) & 66.54 (0.76)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.82 (0.01)} & 0.80 (0.01) & 0.85 (0.01) & 58.39 (1.01)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.77 (0.01)} & 0.74 (0.01) & 0.81 (0.01) & 68.14 (1.30)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.79 (0.01)} & 0.76 (0.01) & 0.82 (0.01) & 64.59 (1.01)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.75 (0.01)} & 0.66 (0.02) & 0.85 (0.01) & 1457.12 (35.00)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.86 (0.01)} & 0.79 (0.02) & 0.93 (0.01) & 1135.22 (49.38)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.72 (0.01)} & 0.62 (0.02) & 0.83 (0.02) & 1536.82 (46.74)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.76 (0.01)} & 0.66 (0.02) & 0.85 (0.01) & 1438.48 (33.83)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.77 (0.01)} & 0.74 (0.02) & 0.80 (0.02) & 17.51 (0.69)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.83 (0.01)} & 0.80 (0.02) & 0.85 (0.02) & 13.42 (0.81)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.76 (0.01)} & 0.73 (0.02) & 0.79 (0.02) & 17.73 (1.15)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.79 (0.01)} & 0.76 (0.02) & 0.81 (0.02) & 15.48 (0.74)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & \textcolor{black}{0.83 (0.02)} & 0.83 (0.02) & 0.84 (0.02) & 24.12 (1.02)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.84 (0.02)} & 0.83 (0.02) & 0.84 (0.03) & 23.95 (1.89)\\
\hspace{1em}KM Decensoring & \textcolor{black}{0.80 (0.02)} & 0.80 (0.03) & 0.81 (0.03) & 27.86 (2.16)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.85 (0.02)} & 0.84 (0.02) & 0.85 (0.02) & 22.04 (1.22)\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_grf_alpha_0.2_small.tex <==
\begin{table}[!h]
\centering
\caption{Caption \label{tab:1}}
\centering
\begin{tabular}[t]{ccc}
\toprule
Method & Estimated Coverage & Mean LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & 0.80 (0.80--0.81) & 567.35\\
\hspace{1em}Naive CQR & 0.81 (0.81--0.81) & 563.05\\
\hspace{1em}KM Decensoring & 0.80 (0.80--0.80) & 576.70\\
\hspace{1em}DR-COSARC & 0.81 (0.81--0.82) & 543.45\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & 0.80 (0.79--0.81) & 20.59\\
\hspace{1em}Naive CQR & 0.82 (0.81--0.83) & 19.56\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.79 (0.78--0.81}) & 20.96\\
\hspace{1em}DR-COSARC & 0.81 (0.79--0.82) & 20.12\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.69 (0.56--0.83}) & 36.38\\
\hspace{1em}Naive CQR & 0.87 (0.81--0.93) & 12.92\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.70 (0.57--0.83}) & 35.96\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.74 (0.63--0.85}) & 28.18\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.78 (0.75--0.81}) & 66.54\\
\hspace{1em}Naive CQR & 0.82 (0.80--0.85) & 58.39\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.77 (0.74--0.81}) & 68.14\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.79 (0.76--0.82}) & 64.59\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.75 (0.66--0.85}) & 1457.12\\
\hspace{1em}Naive CQR & 0.86 (0.79--0.93) & 1135.22\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.72 (0.62--0.83}) & 1536.82\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.76 (0.66--0.85}) & 1438.48\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.77 (0.74--0.80}) & 17.51\\
\hspace{1em}Naive CQR & 0.83 (0.80--0.85) & 13.42\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.76 (0.73--0.79}) & 17.73\\
\hspace{1em}DR-COSARC & 0.79 (0.76--0.81) & 15.48\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & 0.83 (0.83--0.84) & 24.12\\
\hspace{1em}Naive CQR & 0.84 (0.83--0.84) & 23.95\\
\hspace{1em}KM Decensoring & 0.80 (0.80--0.81) & 27.86\\
\hspace{1em}DR-COSARC & 0.85 (0.84--0.85) & 22.04\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_rf_alpha_0.1_small.tex <==
\begin{table}[!h]
\centering
\caption{Caption \label{tab:1}}
\centering
\begin{tabular}[t]{ccc}
\toprule
Method & Estimated Coverage & Mean LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & 0.90 (0.89--0.91) & 403.71\\
\hspace{1em}Naive CQR & 0.91 (0.90--0.91) & 379.64\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.89 (0.89--0.90}) & 406.86\\
\hspace{1em}DR-COSARC & 0.91 (0.90--0.91) & 379.60\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.89 (0.88--0.90}) & 14.48\\
\hspace{1em}Naive CQR & 0.91 (0.90--0.92) & 13.43\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.89 (0.88--0.90}) & 14.55\\
\hspace{1em}DR-COSARC & 0.90 (0.89--0.91) & 14.05\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.83 (0.76--0.90}) & 18.26\\
\hspace{1em}Naive CQR & 0.95 (0.93--0.97) & 4.55\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.83 (0.77--0.90}) & 17.58\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.87 (0.82--0.93}) & 11.45\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.89 (0.88--0.91}) & 43.21\\
\hspace{1em}Naive CQR & 0.91 (0.90--0.93) & 39.45\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.89 (0.87--0.90}) & 44.67\\
\hspace{1em}DR-COSARC & 0.90 (0.88--0.91) & 42.22\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.88 (0.82--0.94}) & 1057.31\\
\hspace{1em}Naive CQR & 0.95 (0.91--0.98) & 662.76\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.86 (0.79--0.92}) & 1117.82\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.88 (0.83--0.94}) & 1012.21\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.88 (0.86--0.89}) & 9.75\\
\hspace{1em}Naive CQR & 0.91 (0.89--0.92) & 7.90\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.88 (0.86--0.90}) & 9.78\\
\hspace{1em}DR-COSARC & 0.89 (0.88--0.91) & 8.19\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & 0.90 (0.90--0.90) & 33.90\\
\hspace{1em}Naive CQR & 0.94 (0.94--0.94) & 19.12\\
\hspace{1em}KM Decensoring & 0.91 (0.91--0.91) & 29.50\\
\hspace{1em}DR-COSARC & 0.93 (0.93--0.93) & 21.33\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_rf_alpha_0.2_large.tex <==
\begin{table}[!h]
\centering
\caption{Performance on seven publicly available data sets of different methods for constructing survival LPBs. All methods utilize the same survival model (rf) and aim for 80\% coverage. Since the performance is evaluated on a censored test set, the coverage cannot be evaluated exactly. Instead, we report empirical lower and upper bounds for the true coverage. Values in parentheses represent twice the standard error. Coverage point estimates that are more than two standard errors below the nominal level are highlighted in red. \label{tab:data-rf-large-alpha0.2}}
\centering
\begin{tabular}[t]{ccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Estimated Coverage} & \multicolumn{1}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4}
Method & Point & Lower bound & Upper bound & LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.77 (0.01)} & 0.74 (0.01) & 0.81 (0.01) & 769.68 (16.40)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.83 (0.01)} & 0.80 (0.01) & 0.86 (0.01) & 666.50 (17.43)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.77 (0.01)} & 0.74 (0.01) & 0.81 (0.01) & 773.25 (18.24)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.79 (0.01)} & 0.76 (0.01) & 0.81 (0.01) & 734.72 (16.56)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.79 (0.00)} & 0.77 (0.01) & 0.81 (0.01) & 23.05 (0.23)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.83 (0.00)} & 0.81 (0.01) & 0.84 (0.01) & 20.83 (0.36)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.79 (0.01)} & 0.77 (0.01) & 0.81 (0.01) & 22.83 (0.37)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.80 (0.01)} & 0.78 (0.01) & 0.81 (0.01) & 22.26 (0.33)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.69 (0.02)} & 0.55 (0.03) & 0.82 (0.02) & 51.01 (7.87)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.87 (0.02)} & 0.82 (0.03) & 0.93 (0.01) & 22.85 (6.81)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.72 (0.02)} & 0.60 (0.04) & 0.84 (0.02) & 46.27 (6.90)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.74 (0.02)} & 0.63 (0.04) & 0.85 (0.02) & 36.86 (5.92)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.78 (0.00)} & 0.74 (0.01) & 0.81 (0.01) & 69.70 (0.80)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.83 (0.01)} & 0.80 (0.01) & 0.86 (0.01) & 60.25 (1.08)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.78 (0.01)} & 0.74 (0.01) & 0.81 (0.01) & 70.17 (1.27)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.79 (0.01)} & 0.76 (0.01) & 0.82 (0.01) & 67.54 (1.02)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.74 (0.01)} & 0.63 (0.02) & 0.86 (0.01) & 1597.23 (40.63)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.87 (0.01)} & 0.79 (0.02) & 0.95 (0.01) & 1100.00 (72.19)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.73 (0.01)} & 0.61 (0.02) & 0.85 (0.02) & 1629.48 (53.68)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.75 (0.01)} & 0.64 (0.02) & 0.87 (0.01) & 1539.17 (43.28)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.74 (0.01)} & 0.68 (0.02) & 0.80 (0.02) & 21.77 (0.83)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.84 (0.01)} & 0.80 (0.02) & 0.88 (0.02) & 14.65 (1.03)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.75 (0.01)} & 0.69 (0.02) & 0.80 (0.02) & 21.17 (1.18)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.77 (0.01)} & 0.72 (0.02) & 0.82 (0.02) & 18.82 (1.15)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & \textcolor{black}{0.82 (0.02)} & 0.81 (0.02) & 0.82 (0.02) & 34.20 (8.65)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.83 (0.02)} & 0.83 (0.02) & 0.84 (0.02) & 33.41 (8.50)\\
\hspace{1em}KM Decensoring & \textcolor{black}{0.80 (0.02)} & 0.79 (0.03) & 0.80 (0.03) & 37.39 (8.30)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.84 (0.01)} & 0.83 (0.02) & 0.84 (0.02) & 30.94 (7.70)\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_rf_alpha_0.2_small.tex <==
\begin{table}[!h]
\centering
\caption{Caption \label{tab:1}}
\centering
\begin{tabular}[t]{ccc}
\toprule
Method & Estimated Coverage & Mean LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.77 (0.74--0.81}) & 769.68\\
\hspace{1em}Naive CQR & 0.83 (0.80--0.86) & 666.50\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.77 (0.74--0.81}) & 773.25\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.79 (0.76--0.81}) & 734.72\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.79 (0.77--0.81}) & 23.05\\
\hspace{1em}Naive CQR & 0.83 (0.81--0.84) & 20.83\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.79 (0.77--0.81}) & 22.83\\
\hspace{1em}DR-COSARC & 0.80 (0.78--0.81) & 22.26\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.69 (0.55--0.82}) & 51.01\\
\hspace{1em}Naive CQR & 0.87 (0.82--0.93) & 22.85\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.72 (0.60--0.84}) & 46.27\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.74 (0.63--0.85}) & 36.86\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.78 (0.74--0.81}) & 69.70\\
\hspace{1em}Naive CQR & 0.83 (0.80--0.86) & 60.25\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.78 (0.74--0.81}) & 70.17\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.79 (0.76--0.82}) & 67.54\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.74 (0.63--0.86}) & 1597.23\\
\hspace{1em}Naive CQR & 0.87 (0.79--0.95) & 1100.00\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.73 (0.61--0.85}) & 1629.48\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.75 (0.64--0.87}) & 1539.17\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.74 (0.68--0.80}) & 21.77\\
\hspace{1em}Naive CQR & 0.84 (0.80--0.88) & 14.65\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.75 (0.69--0.80}) & 21.17\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.77 (0.72--0.82}) & 18.82\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & 0.82 (0.81--0.82) & 34.20\\
\hspace{1em}Naive CQR & 0.83 (0.83--0.84) & 33.41\\
\hspace{1em}KM Decensoring & 0.80 (0.79--0.80) & 37.39\\
\hspace{1em}DR-COSARC & 0.84 (0.83--0.84) & 30.94\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_survreg_alpha_0.1_small.tex <==
\begin{table}[!h]
\centering
\caption{Caption \label{tab:1}}
\centering
\begin{tabular}[t]{ccc}
\toprule
Method & Estimated Coverage & Mean LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & 0.90 (0.90--0.90) & 369.05\\
\hspace{1em}Naive CQR & 0.91 (0.91--0.91) & 351.31\\
\hspace{1em}KM Decensoring & 0.90 (0.90--0.90) & 361.87\\
\hspace{1em}DR-COSARC & 0.91 (0.91--0.91) & 339.93\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & 0.90 (0.89--0.91) & 13.43\\
\hspace{1em}Naive CQR & 0.91 (0.90--0.92) & 12.69\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.89 (0.88--0.90}) & 13.80\\
\hspace{1em}DR-COSARC & 0.90 (0.89--0.91) & 13.17\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.83 (0.75--0.90}) & 22.72\\
\hspace{1em}Naive CQR & 0.94 (0.91--0.97) & 8.91\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.84 (0.77--0.91}) & 20.75\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.86 (0.81--0.92}) & 14.22\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.88 (0.87--0.90}) & 46.04\\
\hspace{1em}Naive CQR & 0.92 (0.91--0.93) & 38.98\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.89 (0.87--0.91}) & 44.98\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.89 (0.88--0.91}) & 43.66\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.85 (0.79--0.92}) & 1197.47\\
\hspace{1em}Naive CQR & 0.95 (0.92--0.98) & 738.45\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.86 (0.79--0.92}) & 1167.58\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.87 (0.82--0.93}) & 1098.76\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.87 (0.85--0.88}) & 9.22\\
\hspace{1em}Naive CQR & 0.91 (0.89--0.92) & 6.93\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.87 (0.86--0.89}) & 8.79\\
\hspace{1em}DR-COSARC & 0.89 (0.88--0.91) & 7.13\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & 0.89 (0.89--0.90) & 21.47\\
\hspace{1em}Naive CQR & 0.94 (0.93--0.94) & 16.92\\
\hspace{1em}KM Decensoring & 0.89 (0.88--0.89) & 22.24\\
\hspace{1em}DR-COSARC & 0.92 (0.91--0.92) & 17.27\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_survreg_alpha_0.2_large.tex <==
\begin{table}[!h]
\centering
\caption{Performance on seven publicly available data sets of different methods for constructing survival LPBs. All methods utilize the same survival model (survreg) and aim for 80\% coverage. Since the performance is evaluated on a censored test set, the coverage cannot be evaluated exactly. Instead, we report empirical lower and upper bounds for the true coverage. Values in parentheses represent twice the standard error. Coverage point estimates that are more than two standard errors below the nominal level are highlighted in red. \label{tab:data-survreg-large-alpha0.2}}
\centering
\begin{tabular}[t]{ccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Estimated Coverage} & \multicolumn{1}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4}
Method & Point & Lower bound & Upper bound & LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.78 (0.01)} & 0.77 (0.01) & 0.79 (0.01) & 736.71 (14.33)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.82 (0.01)} & 0.81 (0.01) & 0.83 (0.01) & 649.62 (15.87)\\
\hspace{1em}KM Decensoring & \textcolor{black}{0.80 (0.01)} & 0.79 (0.01) & 0.81 (0.01) & 690.86 (15.50)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.80 (0.01)} & 0.79 (0.01) & 0.81 (0.01) & 661.78 (16.51)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.79 (0.00)} & 0.77 (0.01) & 0.80 (0.01) & 22.09 (0.25)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.82 (0.00)} & 0.81 (0.01) & 0.83 (0.01) & 19.88 (0.34)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.79 (0.01)} & 0.78 (0.01) & 0.81 (0.01) & 21.53 (0.38)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.80 (0.01)} & 0.78 (0.01) & 0.81 (0.01) & 21.04 (0.31)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.70 (0.02)} & 0.58 (0.03) & 0.82 (0.02) & 57.91 (6.79)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.86 (0.02)} & 0.80 (0.03) & 0.93 (0.02) & 31.61 (5.46)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.72 (0.03)} & 0.60 (0.05) & 0.84 (0.02) & 53.84 (5.76)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.75 (0.02)} & 0.65 (0.04) & 0.85 (0.02) & 41.11 (5.20)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.77 (0.01)} & 0.74 (0.01) & 0.81 (0.01) & 71.64 (0.83)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.83 (0.01)} & 0.81 (0.01) & 0.86 (0.01) & 60.00 (1.15)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.77 (0.01)} & 0.74 (0.01) & 0.81 (0.01) & 71.13 (1.37)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.79 (0.01)} & 0.75 (0.01) & 0.82 (0.01) & 68.86 (1.37)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.72 (0.01)} & 0.59 (0.02) & 0.85 (0.01) & 1789.56 (61.43)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.88 (0.01)} & 0.80 (0.02) & 0.95 (0.01) & 1152.86 (73.90)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.75 (0.01)} & 0.63 (0.02) & 0.87 (0.01) & 1668.70 (62.27)\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.74 (0.01)} & 0.62 (0.02) & 0.86 (0.01) & 1590.80 (43.55)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.75 (0.01)} & 0.71 (0.02) & 0.80 (0.01) & 20.92 (1.02)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.84 (0.01)} & 0.81 (0.02) & 0.88 (0.02) & 13.74 (1.08)\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.78 (0.02)} & 0.73 (0.03) & 0.82 (0.02) & 18.96 (1.23)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.79 (0.01)} & 0.75 (0.02) & 0.82 (0.02) & 17.16 (1.27)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & \textcolor{black}{0.82 (0.01)} & 0.82 (0.02) & 0.83 (0.02) & 34.77 (1.51)\\
\hspace{1em}Naive CQR & \textcolor{black}{0.85 (0.02)} & 0.84 (0.03) & 0.86 (0.03) & 31.91 (3.12)\\
\hspace{1em}KM Decensoring & \textcolor{black}{0.81 (0.02)} & 0.80 (0.03) & 0.82 (0.03) & 36.57 (2.41)\\
\hspace{1em}DR-COSARC & \textcolor{black}{0.84 (0.02)} & 0.83 (0.02) & 0.84 (0.02) & 31.29 (2.28)\\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_data_survreg_alpha_0.2_small.tex <==
\begin{table}[!h]
\centering
\caption{Caption \label{tab:1}}
\centering
\begin{tabular}[t]{ccc}
\toprule
Method & Estimated Coverage & Mean LPB\\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{COLON}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.78 (0.77--0.79}) & 736.71\\
\hspace{1em}Naive CQR & 0.82 (0.81--0.83) & 649.62\\
\hspace{1em}KM Decensoring & 0.80 (0.79--0.81) & 690.86\\
\hspace{1em}DR-COSARC & 0.80 (0.79--0.81) & 661.78\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{GBSG}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.79 (0.77--0.80}) & 22.09\\
\hspace{1em}Naive CQR & 0.82 (0.81--0.83) & 19.88\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.79 (0.78--0.81}) & 21.53\\
\hspace{1em}DR-COSARC & 0.80 (0.78--0.81) & 21.04\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{HEART}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.70 (0.58--0.82}) & 57.91\\
\hspace{1em}Naive CQR & 0.86 (0.80--0.93) & 31.61\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.72 (0.60--0.84}) & 53.84\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.75 (0.65--0.85}) & 41.11\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{METABRIC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.77 (0.74--0.81}) & 71.64\\
\hspace{1em}Naive CQR & 0.83 (0.81--0.86) & 60.00\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.77 (0.74--0.81}) & 71.13\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.79 (0.75--0.82}) & 68.86\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{PBC}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.72 (0.59--0.85}) & 1789.56\\
\hspace{1em}Naive CQR & 0.88 (0.80--0.95) & 1152.86\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.75 (0.63--0.87}) & 1668.70\\
\hspace{1em}DR-COSARC & \textcolor{red}{0.74 (0.62--0.86}) & 1590.80\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{RETINOPATHY}}\\
\hspace{1em}Uncalibrated & \textcolor{red}{0.75 (0.71--0.80}) & 20.92\\
\hspace{1em}Naive CQR & 0.84 (0.81--0.88) & 13.74\\
\hspace{1em}KM Decensoring & \textcolor{red}{0.78 (0.73--0.82}) & 18.96\\
\hspace{1em}DR-COSARC & 0.79 (0.75--0.82) & 17.16\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{VALCT}}\\
\hspace{1em}Uncalibrated & 0.82 (0.82--0.83) & 34.77\\
\hspace{1em}Naive CQR & 0.85 (0.84--0.86) & 31.91\\
\hspace{1em}KM Decensoring & 0.81 (0.80--0.82) & 36.57\\
\hspace{1em}DR-COSARC & 0.84 (0.83--0.84) & 31.29\\
\bottomrule
\end{tabular}
\end{table}

